How Low Can We Go? Pixel Annotation for Semantic Segmentation

How many labeled pixels are needed to segment an image, without any prior knowledge? We conduct an experiment to answer this question. In our experiment, an Oracle is using Active Learning to train a network from scratch. The Oracle has access to the entire label map of the image, but the goal is to reveal as little pixel labels to the network as possible. We find that, on average, the Oracle needs to reveal (i.e., annotate) less than 0.1% of the pixels in order to train a network. The network can then label all pixels in the image at an accuracy of more than 98%. Based on this single-image-annotation experiment, we design an experiment to quickly annotate an entire data set. In the data set level experiment the Oracle trains a new network for each image from scratch. The network can then be used to create pseudo-labels, which are the network predicted labels of the unlabeled pixels, for the entire image. Only then, a data set level network is trained from scratch on all the pseudo-labeled images at once. We repeat both image level and data set level experiments on two, very different, real-world data sets, and find that it is possible to reach the performance of a fully annotated data set using a fraction of the annotation cost.

==> Chapters/backup_01_introduction.tex <==
\section{Introduction}

\begin{figure}[]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.9\linewidth]{latex/ICCV_2021/Figures/Images/main_pipeline.pdf}\\
\end{tabular}
\caption{ Proposed pipeline. Given an image, we pass it through the proposed Pseudo-Optimal Algorithm that estimates ~0.1\% pixels location we should annotate. Using labels only on those pixels, we infer a pseudo label. We can later train a model on an entire dataset using those labels and achieve full supervision results. \daniel{make network block so it won't seem it changes the size}}
\label{fig:teaser}
\end{center}
\end{figure}

Semantic segmentation of images is one of the most useful operations in computer vision. It is used in various applications such as image editing, image understanding, medical image analysis and more. This task is still a challenge especially because of the large variability in image content. Very often, to achieve high quality results, a specialized semantic segmentation training set must be created, which might be a daunting task. But is it really? We wish to shed some light on the annotation process by giving some insights into the amount of work needed to segment an image, and hopefully provide a strong baseline for further research on this subject.

We tackle the question of how much information is needed to create an effective training set for the task of semantic segmentation? A typical approach for annotating a new dataset of images is to rely on standard image annotation tools, such as scribbles to annotate images and semi-automatically segment them. Repeating this process over many images can create a large enough set to train a semantic segmentation network. Still, it is not clear \textbf{where to place the scribbles} in the image, and \textbf{how many scribbles are actually required} to correctly segment an image.

Suppose that you wish to label a new dataset with a limited budget, what are the most "informative" clicks for a given image? We wish to "spend" the budget judiciously to get more from the limited budget. See an overview of our method in Figure~\ref{fig:teaser}.

One can agree that some pixels are more "important" for training than others. A common intuition is to sample around the object boundaries~\cite{ding2019boundary, wang2019boundary, hariharan2011semantic, Yu_2017_CVPR}. However, that notion of importance can change based on the image content and the label image, thus making it hard to generalize. It is also not clear which boundary pixels are important?

% We show systematically the amount and location of the pixels we need to sample in order to reconstruct the entire semantic label image.

To address this, we analyze the number of pixels required to annotate a single image. We use existing semantic segmentation datasets, for which the ground truth is known, and evaluate different methods to sample pixels to serve as annotated ``scribbles''. We use labels only on the selected pixels to train a neural network for segmentation.
In our approach, the user is replaced with an Oracle that determines which pixels to scribble. Such an Oracle-based approach allows us to evaluate different ways to determine how many pixels should be annotated and find their distribution in the image plane. 

Because we train the network to train just a single image, the number of labeled pixels is quite low. We found that, on average, annotating up to $0.1\%$ of the pixels in an image is sufficient to train the network to segment the image successfully. There is no need to pre-train the network on a large training data set beforehand.

Next, we investigate how to extend this approach to the annotation of an entire data set. A na\"ive extension of our findings above would be to annotate $0.1\%$ of the pixels in many images, and use only them to train a network for the entire data set. However, we found that this does not work well, and took a different approach. 

Instead, for each image, we use the single-image-network we trained in the previous step to find and annotate pixels, but use them to create pseudo-labels for the entire image. These pseudo-labels are sufficiently accurate to train a new network for the entire data set. We found that using as little as $30\%$ of the images from the original training set gives good results with little degradation in accuracy compared to training with the full training set. We demonstrate this on two very different types of datasets: the PASCAL VOC 2012 dataset ~\cite{pascal-voc-2012}, a popular instance segmentation benchmark, and Kvasir-SEG ~\cite{jha2020sessile}, a medical imaging binary segmentation set. We make the following contributions:
\begin{itemize}
  \item Propose a plug-and-play single image annotation algorithm that can work with any network architecture.
  \item Suggest a method to quickly annotate an entire data set based on our single-image-annotation approach.
  \item Run extensive experiments to validate our results on two, very different, real-world data sets.
\end{itemize}


% As we wish to estimate the amount of information needed to train a network, without any prior knowledge, we wish to exploit the internal statistics of an image for this matter. We utilize the field of 'Deep Internal Learning', that has seen increasing interest lately \daniel{Add refs? If we want to keep it as a section}, to work on semantic segmentation. 

% \textbf{Contributions.}
% \daniel{A bit copied from the 10\% we don't need - contribution} This work shed some light on semantic redundancies in semantic segmentation, which in turn can be used in various fields (improving interactive segmentation by proposing the important regions to the user, applying more sophisticated training techniques on a sparse supervision to improve explainability, reducing computation cost and labeling efforts). We do it by identifying a subset of pixels that are \textit{informative}, such that knowing them will help recover the entire semantic label image. To the best of our knowledge, this is the first work to suggest a feasible solution to which highly sparse pixels are informative for the task of semantic segmentation.

% \daniel{A bit copied from the 10\% we don't need - contribution} We do not claim algorithmic contributions, but rather demonstrating the existence of pixels redundancies in semantic segmentation across different datasets. However, we hope that our findings can motivate further research into identifying additional redundancies and exploiting them for more efficient models, training or data-collection. Our findings may also be of interest to active learning community, as it provides an upper-bound on the best performance\footnote{\daniel{A bit copied from the 10\% we don't need - footnote} Suppose we discover about the existence of $k$ pixels in an image of size $n >> k$ that contains all of the \textit{information} of the image and can reach at least the same results as using all $n$ pixels. Then if our training procedure cannot reach the full supervision performance after selecting $k$ pixels, we know that there \textit{might} exists a better training procedure, as there exists a subset of size $k$ that can achieve full supervision performance.
% %Suppose we learn about existence of m samples in a dataset of size $n > m$ that can achieve the same test performance as a model trained with all $n$ samples. Then if our active learner cannot reach the full test performance after selecting $m$ samples, we know that there \textit{might} exist a better active learning algorithm, as the ideal subset of size $m$ can achieve full test accuracy
% }.


%-------------------------------------------------------------------------

% \begin{itemize}
%   \item Propose a plug-and-play single image annotation algorithm that can work with any network architecture.
  
%   'easy-to-implement' \daniel{plug and play? we need to emphasize that unlike other papers, our approach is straightforward and easy to validate} generic algorithm for uncovering the most "informative" pixels for the task of semantic segmentation.
%   \item Give a notion of 'Curriculum Learning' in the pixel level.
%   \item Run extensive experiments and validate our results on two, very different, real-world datasets.
%   \item Expand the concept of 'Deep Internal Learning' for semantic segmentation.
%   \item Increase explainability of segmentation networks training by uncovering some insights.
% \end{itemize}


==> Chapters/backup_02_background.tex <==
\section{Related Work}
Various Zero-Shot semantic segmentation solutions exists \cite{kato2019zero, bucher2019zero}, but a common ground is that they use sort of past knowledge and expand it to unseen classes, some in the form of a single image, some with an entire dataset. We, however, are dealing with the amount of information needed and we don't want to assume any prior knowledge of any kind.

Some work explore redundancies of images from an entire dataset. \cite{birodkar2019semantic} explored such redundancies in image classification and found that on 10\% of CIFAR-10 and ImageNet datasets can be ignored and still reach the same performance. While \cite{vodrahalli2018all} analyze relative importance of training images in four datasets of varying complexity and found that in some cases, a small subsample is indeed sufficient for training. However, those datasets are for the task of image classification and are not as challenging as those we chose.

We develop an extension of curriculum learning\cite{bengio2009curriculum}, which was presented by Bengio {\em et al.} by giving a notion of this concept to the pixel-level. Can some pixels be considered more "easy" or "difficult"? 
We show that showing the network pixels of in a defined order improves model's performance. As far as we know, we are the first to investigate such an extension.

\daniel{Need to fill semi \ weakly supervised, active learning, interactive segmentation}.





%-------------------------------------------------------------------------
\subsection{Old Related Work \daniel{Placeholder until we decide what to keep}}
Semantic segmentation networks have made great progress in recent years. There is a plethora of such methods, starting with the work of Shelhamer, Long and Darrel~\cite{FCN}, all the way to current state of the art methods such as DeepLabv3+~\cite{ChenZPSA18}. The literature on the subject is large and we will focus on work most related to ours.

Training these networks requires huge amounts of annotated ground truth data, and while there are some publicly available datasets such as MS-COCO~\cite{MS-COCO} or CityScapes~\cite{Cityscapes} building them requires considerable amount of effort.
The different datasets usually target different domains. This encouraged Lambert {\em et al.}~\cite{LambertLSHK20} to propose MSeg, a composite dataset that unifies semantic segmentation datasets from different domains. The resulting composite dataset enables training a single semantic segmentation model that functions effectively across domains and generalizes to datasets that were not seen during training. 

% Training these networks requires huge amounts of annotated ground truth data. This puts a heavy burden on humans who must annotate every image in order to create the ground truth semantic map. 

In order to reduce the annotation effort, one may use weakly supervised training schemes. For example, Wei {\em et al.}~\cite{Wei_2018_CVPR} use the Class Action Maps~\cite{ZhouKLOT16} to localize image level labels, which is then used to generate a semantic segmentation map. Dai {\em et al.}~\cite{DaiHS15} use Bounding Boxes as weak annotations. The basic idea is to iterate between automatically generating region proposals and training convolutional networks. Later, Hu {\em et al.}~\cite{HuDHDG18} learned how to segment everything through a mixture of a large set of bounding box annotations and a small fraction of mask annotations.

Bearman {\em et al.}~\cite{BearmanRFL16} combine user-provided point clicks with a novel objectness potential in the training loss function of a CNN model. Lin {\em et al.}~\cite{Lin2016ScribbleSupSC} use scribbles to quickly annotate images. Their algorithm is based on a graphical model that jointly propagates information from scribbles to unmarked pixels and learns network parameters. 

Annotating semantic segmentation maps is closely related to interactive image segmentation, where the leading paradigm is user scribbles. This started with the work of Boykov and Jolly~\cite{BoykovJ01}, that was later extended by Rother~\cite{RotherKB04} to treat the problem as a MRF optimization problem. Bai and Sapiro~\cite{BaiS09} use Geodesic distances to solve the problem, and Brady~\cite{Grady06} use the theory of random walks to solve the problem. The scribbles specify pixels that belong to each class and the network infers the label of the rest of the pixels. A recent line of work relies on the power of CNNs to understand what is an object and thus reduce user interactions to just a few clicks~\cite{Xu_2016_CVPR,LiCK18}.

% The methods that require user interaction assume that the user will know how to best provide his input. Take scribbles, for example, different users will be provide 

Our work is related to Active Learning that iteratively selects the most informative samples to label~\cite{Settles}. In one popular variant, uncertainty pool-based active learning, softmax probabilities from the model’s outputs is used to compute entropy as an uncertainty criterion for the future manual annotation~\cite{Gal2017}. Recently, Siddiqui {\em et al.}~\cite{SiddiquiVN20} proposed ViewAL that learns semantic segmentation in multi-view datasets by exploiting viewpoint consistency. This allowed them to use just $7\%$ of the pixels in order to label all pixels in the dataset.
%-------------------------------------------------------------------------


\subsection{Weakly-Supervised Segmentation}
Talk about that most method try to get closer to the full supervised method, while some of them show impressive results, there still exists a gap. We wish to bridge this gap.
%-------------------------------------------------------------------------

\subsection{Deep Internal Learning}
As we wish to answer the question of 'how low can we go?' without any prior knowledge, we train a network at "test" time on the input image itself, without any prior knowledge.
The work of Gandelsman, Shocher and Irani ~\cite{DoubleDIP} also explored binary segmentation without any prior knowledge, however this does not deal with semantic segmentation, nor encode user inputs to refine prediction.
We wish to use the internal information along with an Oracle to reveal some mystery about the amount of information needed to get the semantic segmentation of the input image. \newline

%-------------------------------------------------------------------------
\subsection{Interactive Segmentation}
We can talk about papers that try to simulate the user clicks (where to scribble next). Or to create random strokes. Also talk about the results of interactive segmentation, we require one order of magnitude more supervision (user clicks), but we do not assume any prior knowledge.
%-------------------------------------------------------------------------
\subsection{Active Learning Sampling}
Some papers from recent years on active learning show that using about 10\% of the data they reach not far from fully supervised version on Cityscapes. We can talk about it and emphasize the differences and that our work can be a baseline for upper bound (we know there exists a subset <1\% that can do better with less).


%-------------------------------------------------------------------------



























% ==============================================================
\input{latex/ICCV_2021/Figures/Images/TexFiles/sampled_points_visualization_wide}

\section{Related Work}
%-------------------------------------------------------------------------
Supervision on the task of semantic segmentation usually involves using cross-entropy (CE) term for each labeled pixel on the CNN output map, which involves creating expensive annotations for the entire image.

\paragraph{Weakly-Supervised Segmentation}
To lighten this burden, some Weakly-Supervised approaches were proposed which uses less supervision, from image-level labels~\cite{vernaza2017learning, huang2018weakly} through clicks~\cite{BearmanRFL16}, up to scribbles~\cite{Lin2016ScribbleSupSC, tang2018normalized, wang2019boundary} that used more supervision compared to us (two order of magnitude) while not reaching full-supervision results. While more papers came afterwards to to better utilize the amount of supervision while trying to minimize the gap to reach full-supervision results, we aim to look at the problem differently, by finding the amount and locations of pixels needed in order to reach full-supervision results.

\paragraph{General papers that I don't know where to add - I talk about it also in the 'order' section}
As we aim to find a sparse subset of pixels that can encode all of the information about the label image. Some work explore redundancies of images from an entire dataset. \cite{birodkar2019semantic} explored such redundancies in image classification and found that on common datasets, you can ignore 10\% of the training data, and still reach the same performance. However, this does not apply for dense semantic segmentation, nor handle highly sparse results, as we show that 99.9\% can be ignored for our task.
% While \cite{vodrahalli2018all} analyze relative importance of training images in four datasets of varying complexity and found that in some cases, a small subsample is indeed sufficient for training. However, those datasets are for the task of image classification and are not as challenging as those we chose.

Curriculum Learning was shown by \cite{bengio2009curriculum} to increase networks performance and generalization, by presenting the network with gradually increasing complex examples, and not in random order. While the authors showed it in the \emph{image-level}, we show similar behaviour in the \emph{pixel-level}. Training in a pre-defined order can improve results compared to training without any order, and training in an inverse order produce the lowest results.
Can some pixels be considered ''easier'' or ''harder''? \cite{li2017not} gave a such notion and showed a small improvement in the results. However their measurement is based on the ambiguity of network, they classify a large portion of the image as ''moderate'' or ''hard'' difficulty as well as using additional datasets.
We, on the other hand, can learn without any prior knowledge, for each image separately, give such notation for a highly sparse subset of pixels and show large improvement. As far as we know, we are the first to investigate such an extension.

% \daniel{General papers - delete?}
% Semantic segmentation networks have made great progress in recent years. There is a plethora of such methods, starting with the work of Shelhamer, Long and Darrel~\cite{FCN}, all the way to current state of the art methods such as DeepLabv3+~\cite{ChenZPSA18}. The literature on the subject is large and we will focus on work most related to ours.

% Training these networks requires huge amounts of annotated ground truth data, and while there are some publicly available datasets such as MS-COCO~\cite{MS-COCO} or CityScapes~\cite{Cityscapes} building them requires considerable amount of effort.
% The different datasets usually target different domains. This encouraged Lambert {\em et al.}~\cite{LambertLSHK20} to propose MSeg, a composite dataset that unifies semantic segmentation datasets from different domains. The resulting composite dataset enables training a single semantic segmentation model that functions effectively across domains and generalizes to datasets that were not seen during training. 

% Training these networks requires huge amounts of annotated ground truth data. This puts a heavy burden on humans who must annotate every image in order to create the ground truth semantic map. 


%-------------------------------------------------------------------------
% In order to reduce the annotation effort, one may use weakly supervised training schemes. For example, Wei {\em et al.}~\cite{Wei_2018_CVPR} use the Class Action Maps~\cite{ZhouKLOT16} to localize image level labels, which is then used to generate a semantic segmentation map. Dai {\em et al.}~\cite{DaiHS15} use Bounding Boxes as weak annotations. The basic idea is to iterate between automatically generating region proposals and training convolutional networks. Later, Hu {\em et al.}~\cite{HuDHDG18} learned how to segment everything through a mixture of a large set of bounding box annotations and a small fraction of mask annotations.

% Bearman {\em et al.}~\cite{BearmanRFL16} combine user-provided point clicks with a novel objectness potential in the training loss function of a CNN model. Lin {\em et al.}~\cite{Lin2016ScribbleSupSC} use scribbles supervision on ~$3\%$ of the pixels to quickly annotate images. Their algorithm is based on a graphical model that jointly propagates information from scribbles to unmarked pixels and learns network parameters. We, however, use less supervision (two order of magnitudes) and reach full-supervision results.

%-------------------------------------------------------------------------
\paragraph{Interactive Segmentation}
In interactive segmentation, the user can annotate the binary target object with scribbles. Common approaches \cite{Xu_2016_CVPR,li2018interactive,agustsson2019interactive,lin2020interactive} differ in the amount of user-clicks needed, generalization to unseen datasets as well as amount of supervision needed for training. We on the other hand, are interested in multi-label segmentation, without any prior knowledge. Moreover, while interactive segmentation rely on trained models refinement at inference time, we train our network \emph{from scratch} at inference time.
Li {\em et al.} \cite{li2018interactive} reached $85\%$ and $90\%$ mIoU scores on Pascal-VOC using 7 and 10 clicks, respectively, by learning binary predictions for each class, and refining the results from the user clicks. Recently, \cite{lin2020interactive} showed that it is possible to do it with 3 and 4 clicks, while relying on large datasets training. Although we do not aim to compete with these methods, as we aim to find redundancies in image segmentation, we saw that, without any prior knowledge \daniel{except imagenet pretraining}, we need 15 and 20 clicks to reach the same thresholds.

% Annotating semantic segmentation maps is closely related to interactive image segmentation, where the leading paradigm is user scribbles. This started with the work of Boykov and Jolly~\cite{BoykovJ01}, that was later extended by Rother~\cite{RotherKB04} to treat the problem as a MRF optimization problem. Bai and Sapiro~\cite{BaiS09} use Geodesic distances to solve the problem, and Brady~\cite{Grady06} use the theory of random walks to solve the problem. The scribbles specify pixels that belong to each class and the network infers the label of the rest of the pixels. 

% A recent line of work relies on the power of CNNs to understand what is an object and thus reduce user interactions to just a few clicks~\cite{}.
% \shai{Give more details on these methods and also cite the CVPR'20 paper.}

% To put things in context, recent work on interactive image segmentation achieves lower pixel count. Li {\em et al.} \cite{li2018interactive} reached $85\%$ and $90\%$ mIoU scores on Pascal-VOC using 7 and 10 clicks, respectively, by learning binary predictions for each class, and refining the results from the user clicks. We, on the other hand, require about twice the number of clicks (roughly $15$ and $20$ clicks, respectively). Recently, \cite{lin2020interactive} further showed impressive results using less than 4 user clicks, however they also trained their model using a dataset that is similar to the one used for testing.

% We do not compete with these methods, as we aim to answer a different question. Our goal is to determine how many clicks are required to train a network from scratch. The work rely on trained models on large datasets, while in inference time, they only refine the output using the user clicks. We, on the other hand, train our network \emph{for scratch} for each image, at inference time, without any progressive learning. 
% Another important distinction between us and prior work is that they focus on foreground/background segmentation, whereas we consider multi-label segmentation tasks. This automatically increases the number of required point clicks.

%-------------------------------------------------------------------------
\paragraph{Active Learning Sampling}
Our work is related to Active Learning that iteratively selects the most informative samples to label~\cite{Settles}. In one popular variant, uncertainty pool-based active learning, softmax probabilities from the model’s outputs is used to compute entropy as an uncertainty criterion for the future manual annotation~\cite{Gal2017}. Recently, Siddiqui {\em et al.}~\cite{SiddiquiVN20} proposed ViewAL that learns semantic segmentation in multi-view datasets by exploiting viewpoint consistency. This allowed them to use just $7\%$ of the pixels in order to label all pixels in the dataset. 
It was shown by \cite{casanova2020reinforced} that using labels of 9\% of CityScapes~\cite{Cityscapes} dataset can achieve full-supervision results, by labeling only small informative image regions. \daniel{We show competitive results on ADE20K\cite{zhou2017scene} dataset while using almost two order of magnitudes less supervision, see supplementary for more information.}

%-------------------------------------------------------------------------
\paragraph{Zero Shot Semantic Segmentation}
% Various Zero-Shot semantic segmentation solutions exists \cite{kato2019zero, bucher2019zero}, but a common ground is that they use sort of past knowledge and expand it to unseen classes, some in the form of a single image, some with an entire dataset. We, however, are dealing with the amount of information needed and we don't want to assume any prior knowledge of any kind. \shai{Expand on what these methods do}
While Zero-Shot segmentation addresses the problem where not all classes are represented in the training examples. Learning is usually done by transferring knowledge from training examples to unseen classes, as shown by \cite{ bucher2019zero} that generated synthetic training data for unseen classes. However, we are interested from learning without any prior knowledge, at inference time.
\daniel{This is important: }It was shown by ~\cite{gandelsman2019double} that it is possible to segment an image, without any prior knowledge, however this does not deal with multi-label segmentation, nor encode user inputs to refine prediction.


% \paragraph{Deep Internal Learning}
% As we wish to answer the question of 'how low can we go?' without any prior knowledge, we train a network at "test" time on the input image itself, without any prior knowledge.
% The work of Gandelsman, Shocher and Irani ~\cite{gandelsman2019double} also explored binary segmentation without any prior knowledge, however this does not deal with semantic segmentation, nor encode user inputs to refine prediction.
% We wish to use the internal information along with an Oracle to reveal some mystery about the amount of information needed to get the semantic segmentation of the input image. \newline

% \shai{Is Deep Internal Learning really relevant to our work?}




==> Chapters/backup_03_method.tex <==
\section{Method}

\section{Method}

\subsection{Motivation}
Giving an image and the corresponding semantic label image, one can ask how many information is needed to successfully create the entire label image? If we were given every second labeled pixel, could we restore the entire label image? What about every four labeled pixel? To uncover the label redundancies, it is important to analyze each image independently from any other prior information. To this end we are interested in an upper bound of the amount of labeled pixels needed in order to successfully\footnote{see section ~\ref{What_is_a_good_segmentation_image} for further explanation on how we define a successful result} restore the label image.


\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.9\linewidth]{latex/CVPR_2021/Images/Method/Redundancy_Algo_example_mine.png} \\
\end{tabular}
\caption{Algorithm pipeline. In each iteration we select the next most informative point. \daniel{placeholder if we decide to add similar pipeline for the new sampling method}}
\label{fig:method::algo}
\end{center}
\end{figure}
%-------------------------------------------------------------------------
\subsection{Pseudo Optimal Algorithm}
\textbf{Problem statement}   Given an Image I, segmentation label image GT, untrained network N, reward R (pixel accuracy/ mean IOU). We seek the find the minimal amount of pixels the network N can be trained on, to maximize the reward between the network prediction, N(I), and the GT. We define the sampled pixels in a binary image m, see equation ~\ref{formula_objective_function}.
% \[m=\{0,1\}^n, \textrm{n is the number of pixels in the image}\]
% \[ S^*= \underset{min_{\|m\|^1}}{\text{max R (GT, N(I) )}, \textrm{s.t. N is trained over } GT \odot m} \]


\[m=\{0,1\}^n, \textrm{n is the number of pixels in the image}\],
\begin{equation} \label{formula_objective_function}
\begin{aligned}
m^*= & \min_{\|m\|^1}\max{R(GT, N(I))}, \\
& \textrm{s.t. N is trained over } GT \odot m
\end{aligned}
\end{equation}

Given a single image, we want to find a minimal subset of pixels that is sufficient to train a {\em single image} network to predict the correct pixel labels for the entire image. The idea is to train a segmentation network on the input image using only the labels of the subset of pixels.
%This means that we back-propagate gradients only on the selected pixels using standard cross-entropy loss. 

The result (Reward) of the trained network prediction compared to the ground truth will give us an estimation for the performance of annotating just the selected subset of pixels. 

We need to address two questions. First -- how many pixels (or what percent from all pixels) we need to use to correctly segment the image? and second -- which pixels we need to choose to achieve best results? Assume that we have an Oracle that can answer the second question, i.e., given a number $k$, the Oracle will tell us the \emph{optimal} $k$ pixels to sample from the image (along with their GT classification) to achieve the best segmentation results. Then, the first question can be answered by simply sweeping through all possible $k$ values from 1 to the number of pixels in the image. The problem is, that we do not have such an Oracle.
The brute-force solution is to test all $k$ possibilities, meaning that if we have $n$ pixels in the image, we will have to check all combinations which is $n^k, \text{for } 0 \leq k\leq n$, which is of course not possible.

We take an approach in which the entire label image is known to an Oracle, and the user is allowed to "ask" the Oracle for the label of a specific pixel. Our objective was to maximize the reward (score metric), in our case we chose it to be the standard mean IOU score between the trained network output and the ground truth label image.

We devise a simple greedy algorithm that we call \emph{pseudo-optimal} because it approximates the Oracle's work. The algorithm uses the known ground-truth segmentation mask to judiciously increase the amount of labeled pixels in an iterative manner as follows: 

 \begin{algorithm}
 \caption{PseudoOptimalSample($I, M, k$)}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE Image $I$ \& Segmentation mask $M$, Scalar $k$
 \ENSURE  Selected set of pixels to use for training
  \STATE Initialize segmentation network \label{op::initialize_network}
  \STATE pick a random pixel $p \in I$
  \STATE $S = \{p\}$
  \REPEAT
  \STATE Train network with labels of $S$ \label{op::training}
  \STATE Segment $I$ using current network to get $L$
  \STATE Compute normalized weight map $W$ as the distance transform over the largest misclassified region belonging the label of the lowest IOU score \label{op::create_weight_map}
  \STATE Sample the next pixel(s) $q$ by weighted random sampling using $W$ \label{op::weighted_random_sampling}
  \STATE $S = S \cup \{q\}$
  \UNTIL{$|S| \geq k$}
   \RETURN $S$ 
 \end{algorithmic} 
 \label{algo:pseudo_sample}
 \end{algorithm}

The idea of the algorithm is to iteratively enlarge the set of sampled pixels $S$ for training, until we reach the desired number $k$. One can replace the proposed sampling method with his own.

Each pixel is selected in a greedy manner by choosing it randomly using several criteria : it should be with a label of the lowest IOU score class, it should be of the largest misclassified connected component, it should be as distant as possible from the correctly classified pixels. 
To answer all of the above criteria we use standard OpenCV functions (cv2.connectedComponentsWithStats and cv2.distanceTransform).

This is done by computing a weight map $W$, as stated in step ~\ref{op::create_weight_map} of algorithm ~\ref{algo:pseudo_sample}, using the above criteria and selecting the next pixel by weighted random sampling. 
The motivation for the above criteria is that information will bubble to nearby misclassified pixels, thus sampling the "center" pixel will effect more pixels. Also, sampling the class corresponding to the lowest IOU score will suppose to effect more pixels related to this class, thus improve the overall mean IOU score.
Note that this algorithm must use the ground truth segmentation to compute the misclassified pixels - hence its ``Oracle'' abilities. 
\daniel{I can add a block diagram visualizing the sampling process.}

We can expand the sampling algorithm to pixel accuracy, by changing a few lines. Note that we can replace the way we compute the weight map $W$ with a different calculation that maximizes the pixel accuracy by sampling the center pixel of the largest misclassified region.

\textbf{Main Results} 
We evaluated the methods on two dataset from different domains: Pascal VOC 2012 and Kvasir-SEG.
Pascal VOC semantic segmentation contains 20 classes and has 1464 images for training and 1449 for validation, the validation set is used for testing.
Kvasir-SEG is a medical binary segmentation dataset for polyp segmentation. It contains 1000 images, we randomly selected 800 images for training and 200 for testing.
We compute the value $k$ as a percentage of the number of pixels in the image and compared various sampling rates other than $0.1\%$. For each sampling rate, we ran algorithm ~\ref{algo:pseudo_sample} on the entire train set. Figure~\ref{fig:miou_different_rates} shows the mean IOU score and variance on all train set images of the datasets for different percentage of sampling.
First, as can be seen, even though our pseudo-optimal algorithm is not a real Oracle, it succeeds in selecting the right pixels to guide the segmentation network. 

Second, our experiments show that using about $200$ pixels, or roughly $0.1\%$ out of a $200,000$ pixel image, is enough to produce results that approach those available when training with all the pixels in an image.  
Figure~\ref{fig:with_and_without_imagenet} shows the mean IOU scores for different sampling rates, justifying why we used a sampling rate of $0.1\%$ with our pseudo-optimal algorithm.
We conclude that $0.1\%$ sampling rate per-image can reach around 99.5\% in IOU score over the entire set.

It is important to note that using simple random sampling of pixels, as well as other possible heuristics (as we will show in Section~\ref{sec:classic_method}), do not achieve compatible results. 
Results can be seen at Table ~\ref{tab:different_sampling_methods_classic}.


\textbf{Location of Selected Pixels}  Visually examining the spatial locations of the sampled points across the images showed conclusively that most of the points lay on boundaries of the objects (according to the ground truth label image). From this we conclude that the common intuition to sample in the proximity of the object boundaries does hold. However, we further show which pixels are more important. We can also note that using a classic method of sampling around the object boundaries did not produce good results, even when fused with grid sampling to cover more areas. We can attribute it to the fact that it is not clear in advance which edge pixels are important and where exactly we should sample the edge pixels, closer or farther from the edge. We argue that all of this is highly depended on the state of the network.  

%-------------------------------------------------------------------------
\subsection{What Is a Good Segmentation Image} \label{What_is_a_good_segmentation_image}
We can ask the question of 'what is a good segmentation image?'. Meaning that, when will define our result as adequate? Pixel accuracy of 100\% can sometimes require a lot of information (e.g. user clicks), with small contributions to the final result. We can see some in Figure~\ref{fig:with_and_without_imagenet} that most of the \emph{reward} is achieved in just a small number of clicks (e.g. 0.1\%), while adding more clicks (e.g. 0.2\%) contribute little to the final result. 

We chose to define a good segmentation image as such that will encode all of the information needed for the downstream task. Meaning that, if our objective is to train a network for semantic segmentation, we define a good segmentation image as such that if we train the network using the above image, it will produce the same results, refer to Table ~\ref{tab:dataset_level_training} to further emphasize this point by showing performance of such downstream task trained with various levels of supervision.

%-------------------------------------------------------------------------
\subsection{Pixel-Level Curriculum Learning}
If we adopt a communication theory point of view perspective, we wish to formalize the sampling points as such that if the receiver of the points will train a network the same way, he will get the same results, without having the need to know the random weights of the original network.
%State differently
Given the set of points $S$ produced by Algorithm ~\ref{algo:pseudo_sample} with a reward $R$, we want to check if we train a new network using the same $S$, will we receive the same $R$?
Meaning that, we wish to check if the results are repetitive, in the sense that it will produce the same result over and over again, with little variance as possible. We want to check whether a new network can produce a close enough output using the sparse label $S$ without being depended on the network parameters random initialization.
\daniel{We need to make sure it's clear we take the set $S$ and run it again in the correct order}
We also seek to find whether the order of the point matters to the overall network prediction.
As we compute the sampling mask $S$ iteratively, we keep the order of the sampled points. To this end, we use the above order to propose a curriculum based approach in the pixel domain. 

We found that the pixel order matters. We follow similar path as in curriculum learning and conduct explore four training options:
\begin{enumerate}
\item{\bf Entire Mask} Train on all of the pixels without any consideration to the order. In this configuration we compute the loss on the entire labeled pixels, and repeat the forward-backward for 400 iterations.
\item{\bf Correct order} Train the network in the same order as the pixels were added. Meaning that, in each iteration we add the current pixel(s) to the sampling mask and compute the loss only on the pixels defined in the mask.
\item {\bf Random order} Train the network in a random order which is different than the order the pixels were added.
\item {\bf Reverse order} Train the network in the inverse ordering of the order they were added. This could be thought of as a variant of anti-curriculum ordering, instead of starting from the ``easy'' pixels, we start from the ``hard'' ones.
\end{enumerate} 

We ran this experiment for all train images in the datasets. The results summarized in Table~\ref{tab:training_order_results} indicate that order matters. Training in the correct order yields the best score with the lowest variance.
Changing hyper-parameters did not produce better results, thus, we conclude that the order matters.
Training in reverse order results in lowest score, and larger variance, given similar results as shown by \cite{bengio2009curriculum}, in the \emph{pixel-level}.
We can also observe that if the correct order is unknown, the second best option is to train with the entire mask at once.
Figures~\ref{fig:orderoTraining_all} and ~\ref{fig:results::different_training_with_without_imagenet} also demonstrates the numerical results visually:  the network prediction is more smooth and accurate when training in the correct order. This is sometimes hard to see in the IOU scores but is noticeable when you observe the results.
We note that even for a single image, repeating the same experiment (given the points and their order, training networks with different order) again and again, resulted in all cases, except the greedy order, large variance in the output. Using the optimal points and training a new network (randomly initialized), resulted in almost the same score and very low variance \daniel{slide 180 in the ppt}. 
We can think about it as a variant for the 'lottery ticket hypothesis', but for the order. We argue that there exists an order that will produce optimal results compared to other training order or procedures. \daniel{should keep it? here?}

\begin{figure}[]
\begin{center}
\begin{tabular}{c c}
\includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Pascal-VOC distribution_different_training_procedures_single_plot.png}& \includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Kvasir-Seg distribution_different_training_procedures_single_plot.png}\\
\end{tabular}
\caption{.}
\caption{Distribution of IOU scores over Pascal VOC train set, for different training options, averaged across all Pascal-VOC and Kvasir-Seg training sets. \daniel{This is with ImageNet, I can show also without}}
\label{fig:method::order_of_training}
\end{center}
\end{figure}



\begin{table}
\begin{center}
\begin{tabular}{l c c}
Method & IOU Mean[\%] $\uparrow$ & IOU Variance $\downarrow$ \\
\hline
Correct Order & \textcolor{blue}{99.76} \textbackslash \textcolor{red}{99.53} & \textcolor{blue}{0.79} \textbackslash \textcolor{red}{0.33} \\
Entire Mask &  \textcolor{blue}{94.79} \textbackslash \textcolor{red}{98.48} & \textcolor{blue}{5.92} \textbackslash \textcolor{red}{2.9} \\
Random Order & \textcolor{blue}{94.69} \textbackslash \textcolor{red}{92.1} & \textcolor{blue}{7.09} \textbackslash \textcolor{red}{6.46} \\
Reverse Order & \textcolor{blue}{81.06} \textbackslash \textcolor{red}{63.49} & \textcolor{blue}{12.52} \textbackslash \textcolor{red}{11.17} \\
\hline   
\end{tabular}
\end{center}
\caption{Various training options and their corresponding mean and variance IOU scores, across all \textcolor{blue}{Pascal-VOC} \textbackslash \textcolor{red}{Kvasir-Seg} training sets.}
\label{tab:training_order_results}
\end{table}

\input{latex/CVPR_2021/Images/Experiments/order_of_training_inference}


%-------------------------------------------------------------------------
\subsection{Dataset-Level Training}
Equipped with the single-image-network tool, we turn to dataset level training. A na\"ive extension of our approach is to annotate a few pixels in every image and then train a network at once on all images with these annotations. However, we have found that this does not work well. Training with just $0.1\%$ pseudo-optimal annotated pixels of $100\%$ of the training set yields decrease of \~{}25\% compared to the one achieved using full supervision.

Instead, we take a different approach. For each image, we use the single-image-network method of pseudo-optimal sampling and segmenting the image, and use the final segmentation results as pseudo-labels for the entire image. Then, we use these pseudo-label maps on a subset of the training set to train a full segmentation network.
Here again, we try to measure how many images are enough to train the segmentation network without severely degrading the results. To avoid bias in the mean IOU calculations, we select images from the dataset for our experiment in such a way that preserves the distribution of classes found in the full training dataset.

We report the results in Table~\ref{tab:dataset_level_training} as a function of two variables, the percentage of training set size and the supervision percentage per image. We wish to emphasize and further push previously seen results \cite{bellver2019budget}, that we need less data to reach the same results.
We find that training with pseudo-labels works much better than simple na\"ive sparse label map training, and is very close in performance to training with the true segmentation. We conclude that, on average, sampling $30\%$ of the images in the training set and using their pseudo-labels often suffices, and using 50\% of the data we reach the same results as using the entire labeled training set. These results are similar on the Pascal VOC and Kvasir-SEG datasets. \daniel {update text after updating table results.}

%-------------------------------------------------------------------------

\paragraph{ Daniel changes to add formula}
We define segmentation network $N$, learned weights $W$, label image $Y$, we use the standard Cross-Entropy(CE) loss and reward function $R$ which is the mean IOU score.
While it is common practice to train a segmentation networks using the entire label image as in Equation~\ref{formula_objective_function_orig}, we chose to define the problem differently as stated in Equation~\ref{formula_objective_function_ours}, as finding the "minimal" mask that will output a close enough score. We train the network only on the pixels defined by the mask $S$, but we evaluate performance compared to the entire label image.


\begin{equation}
\begin{aligned}
\hat{L} = N(I;W) ; Loss = CE(\hat{L}, L) ; R=mIOU(\hat{L},L)
%m^*= & \min_{\|m\|^1}\max{R(GT, N(I))}, \\
%& \textrm{s.t. N is trained over } GT \odot m
\end{aligned}
\label{formula_objective_function_orig}
\end{equation}

\[m=\{0,1\}^n, \textrm{n is the number of pixels in the image}\],

\begin{equation}
\begin{aligned}
\hat{L} = {} & N(I;W) ; L = CE(\hat{L}, L \odot S) ; R=mIOU(\hat{L},L) \\
& S^*= \min_{\|S\|^1}{max Reward}
%m^*= & \min_{\|m\|^1}\max{R(GT, N(I))}, \\
%& \textrm{s.t. N is trained over } GT \odot m
\end{aligned}
\label{formula_objective_function_ours}
\end{equation}



==> Chapters/backup_05_experiments.tex <==
\section{Experiments}
\subsection{Technical Information - Single Image}
We validate that our results hold over several different segmentation architectures, but we will show our results on DeepLabV3+ \daniel{add ref} as it is more widely used and better encode spatial information \daniel{don't really have any justification to it}. We used output stride of 16, resnet101 as the backbone, while all parameters are randomly initialized \daniel {except backbone when using ImageNet}. We use standard Cross-Entropy (CE) loss on the labeled pixels, Adam optimizer with learning-rate of 2e-4 and weight decay 1e-4.
As we have a highly sparse label image, we wish to extract the most of what we are given by the Oracle, this is why step ~\ref{op::training} in Algorithm~\ref{algo:pseudo_sample} consist of several iteration of forward-backward, we set it to 10.
Note that we can sample more than one pixel in each iteration for speedup purposes, as stated in step ~\ref{op::weighted_random_sampling}. We saw that sampling $5$
pixels instead of a single pixel in each iteration of the algorithm, results in little degradation in overall performance.

Our runtime is depended on the image size, and the number of forward-backward iterations and the batch size. On average, it takes around $5$ minutes per image \daniel {can take 1 min with optimizations} on a standard GPU (GTX 1080 Ti).
We can see from Figure~\ref{fig:with_and_without_imagenet} that our method quickly converges without priorly been trained on the task of semantic segmentation or on the data itself \daniel{meaning that just after ~0.02-0.05\% we have a high 'enough' score}.

We tested the proposed algorithm on subset of images from other datasets like ADE and Cityscapes that showed promising results (more than an order of magnitude less supervision from recent reported papers \daniel{add ref if we decide to keep}, while reaching full supervision results). Further results will be in the supplementary \daniel {remove?}.

Note that one can alter the proposed algorithm to match one's own score function and we believe that our results will still hold. We checked various sampling methods and kept the one that showed better results (faster and better convergence).

\input{latex/CVPR_2021/Images/Experiments/sampled_points_visualization}

\subsection{Rethinking ImageNet Pre-Training}
Inspired from recent papers ~\cite{he2019rethinking, zoph2020rethinking}, we set to check the importance of ImageNet pre-training. We repeated the single image experiment but we used a randomly initialized backbone (meaning that all network parameters were randomly initialized). We saw that the gap in the reward is smaller than imagined, and even in low-data regime it is possible to start training all of the network parameters without any prior knowledge of any kind on the objective task or image. We can see a comparison in Figure~\ref{fig:with_and_without_imagenet}. Although the graphs can seem with a small gap, the is quite a difference visually, as the label map is much more "noisy" (less sharp boundaries). Also, the importance of training in the correct order receives further boost, as can be seen in Figure~\ref{fig:results::different_training_with_without_imagenet}.

\begin{figure}[t!]
\begin{center}
\begin{tabular}{c c}
\includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Pascal-VOC_With_and_Without_ImageNet.png}& \includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Kvasir-Seg_With_and_Without_ImageNet.png}\\

\end{tabular}
\caption{Final mIOU scores for different sampling rates, when using the Pseudo-Optimal Algorithm, with and without ImageNet pretraining, averaged across all Pascal-VOC and Kvasir-Seg datasets. \daniel{waiting for results on Kvasir, placeholder}}
\label{fig:with_and_without_imagenet}
\end{center}
\end{figure}

\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.9\linewidth]{latex/ICCV_2021/Figures/Images/results_different_training_with_and_without_imagenet.png} \\
\end{tabular}
\caption{Network prediction on a single image from Pascal-VOC using different training techniques and with/without ImageNet. Upper row with ImageNet, lower row is without ImageNet. The images are, from left to right: 'correct order', 'entire mask', 'random order', 'reverse order'. \daniel{Will make the plot nicer of we chose to keep it}}
\label{fig:results::different_training_with_without_imagenet}
\end{center}
\end{figure}


\subsection{Why 0.1\%?}
How many pixels are needed to correctly label an image? We can "stop" when we restored the label image perfectly, or we can define the stopping criterion in such a way that training a network in the dataset level won't result in results degradation.
We set to answer this question by ruining our algorithm with a large enough user-clicks threshold, such that we can examine when we reach saturation. Those results can be shown in Figure~\ref{fig:miou_different_rates}.
From the results we can see that around 0.05-0.1\% is enough to reach near perfect label map results. We can also see that most of the reward is given in the first user-clicks, and the latter clicks are used for refinements.

\begin{figure}[]
\begin{center}
\begin{tabular}{c c}
\includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Pascal-VOC_Why_0_1_With_ImageNet.png}& \includegraphics[width=0.45\linewidth]{latex/ICCV_2021/Figures/Images/Kvasir-Seg_Why_0_1_With_ImageNet.png}\\

\end{tabular}
\caption{Final mIOU scores for different sampling rates, when using the Pseudo-Optimal Algorithm, with ImageNet pretraining, averaged across all Pascal-VOC and Kvasir-Seg datasets. \daniel{add without ImageNet?}}
\label{fig:miou_different_rates}
\end{center}
\end{figure}

\subsection{Dataset-Level Training}
We used our pseudo labels created using Algorithm~\ref{algo:pseudo_sample} and trained a DNN on those labels. As we showed the resulting pseudo labels reach high mean IOU score, even when using less supervision than reported. We wanted to further emphasize what is a sufficient image segmentation. As discussed in section ~\ref{What_is_a_good_segmentation_image} we trained our DNN on labels produced from different levels of supervision. We can see the results in Table~\ref{tab:dataset_level_training}. From the results we can infer, that we can reach similar performance as the fully supervised version, while using a fraction of the supervision.
For Pascal VOC, we trained our network on the train set and tested it on the validation set without using other datasets for augmentations, we believe that it will not change the correctness of our results.



\begin{table}[]
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|}\hline
\diagbox[width=11em]{[\%] Dataset\\Supervision}{[\%] Pixels\\Supervision}&
  0.1 & 0.2 & 100\\ \hline
10\% & \textcolor{blue}{68} \textbackslash \textcolor{red}{78} & \textcolor{blue}{68} \textbackslash \textcolor{red}{78} & \textcolor{blue}{68} \textbackslash \textcolor{red}{78} \\ \hline
30\% & \textcolor{blue}{70} \textbackslash \textcolor{red}{81} & \textcolor{blue}{70} \textbackslash \textcolor{red}{81} & \textcolor{blue}{70} \textbackslash \textcolor{red}{82} \\ \hline
50\% & \textcolor{blue}{53} \textbackslash \textcolor{red}{68} & \textcolor{blue}{70} \textbackslash \textcolor{red}{85} & \textcolor{blue}{73} \textbackslash \textcolor{red}{88} \\ \hline

\end{tabular}
\end{center}
\caption{Comparing models performance [\% mIOU] on test set trained on a subset of images and subset of supervision per image (0.01\%-100\%, a.k.a full supervision). Results are shown on two datasets \textcolor{blue}{Pascal-VOC} \textbackslash \textcolor{red}{Kvasir-Seg}. Fully supervised version (with 100\% of the data) reaches 73\% on Pascal and 88\% on Kvasir. \daniel{Placeholder. Do it only for ImageNet? can do without also, but it will be more experiments to run, I think with ImageNet is more important as it's a dataset level, not single image.}}
\label{tab:dataset_level_training}
\end{table}


\subsection{Using Trained Models}
We can expand our tests for trained models. By asking how many user-clicks are needed to reach satisfying results? We can run our proposed algorithm on trained models and see that we using little user guidance can reach good results. We quantify the gap between a trained network and randomly initialized network, we can see in Figure~\ref{fig:results::trained_model_performance} that this gap can sometimes be not significant.
Still, it is of course better to use a trained network. 
\daniel{Try to show if we are competitive with interactive segmentation networks?}

\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.9\linewidth]{latex/ICCV_2021/Figures/Images/trained_model_performance_pascal.png} \\
\end{tabular}
\caption{Number of clicks needed using a trained model on Pascal train set, evaluated on test set. \daniel{placeholder- old graph, and only on Pascal, should also on Kvasir?}}
\label{fig:results::trained_model_performance}
\end{center}
\end{figure}

\subsection{Classic Sampling Methods} \label{sec:classic_method}
We evaluated the following techniques for sampling $K$ pixels.
\begin{enumerate}
    \item {\bf Random} Randomly select $K$ pixels.
    \item {\bf Uniform} Split the image into a grid with $K$ tiles and sample a pixel randomly from each tile.
    \item {\bf Edge} Find all edge pixels in the image and sample $K$ pixels.
    \item {\bf SLIC} Use SLIC~\cite{AchantaSSLFS12} to split the image into $K$ segments and sample a pixel randomly from each segment.
    \item {\bf Geodesic} Use geodesic distance to sample $K$ pixels. We iteratively select the most distant pixel according to the geodesic distances on the current selected pixels.
    \item {\bf Pseudo Optimal} Use Active Learning. We iteratively sample misclassified pixels and retrain the network on the sampled pixels.
\end{enumerate}

We have tried each sampling technique with a varying number of pixels and report the results in Table~\ref{tab:different_sampling_methods_classic}.
% Figure~\ref{fig:imageSampling} shows the different methods. 

We draw a number of observations from this experiment. First, we observe that {\bf Edges} give the worst results with mean IoU of $42.6\%$ and quite a large variance of $18.3$. The second best method is {\bf SLIC} with mean IOU of $84.1\%$ but again with a very large variance. The best results are obtained by {\bf Pseudo Optimal} with mean IOU of $99\%$ and a fairly low variance.


\begin{figure}[htb!]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.9\linewidth]{latex/CVPR_2021/Images/Experiments/Pascal_dataset/Different_Random_Sampling_Rates1.pdf} \\
\end{tabular}
\caption{IOU scores Vs. Percentage of points sampled randomly on a specific image from Pascal-VOC. \daniel{can be seen as the motivation for our pseudo optimal algorithm. Maybe we should put all classic analysis in the supplementary}}
\label{fig:results::random_sampling}
\end{center}
\end{figure}

We experimented with random sampling by created a random sampled mask at different rates and trained a network using labels only defined by the mask and log the resulting mean IOU score. We repeated the experiment several times, result can be shown on Figure ~\ref{fig:results::random_sampling}.

Sampling around the edges (or a mixture with random/grid sampling to cover more areas), did not produce adequate results (need an order of magnitude more supervision and can even fail, it's depended on the image and labels content).

\begin{table}
\begin{center}
\begin{tabular}{l c c}
Method & Mean IOU[\%] & IOU Variance\\
\hline
Random  & 80.4\% & 14.3\% \\
Uniform & 83.4\% & 13.1\% \\
Edge    & 42.6\% & 18.3\% \\
SLIC    & 84.1\% & 12.2\% \\
Geodesic  & 80.1\% & 12.8\% \\
Pseudo Optimal  & 99.76\% & 0.79\% \\
\hline   
\end{tabular}
\end{center}
\caption{Pascal VOC train set mean IOU scores and variance, using different sampling methods, for sampling rate of 0.1\%.}
\label{tab:different_sampling_methods_classic}
\end{table}

%-------------------------------------------------------------------------


==> Chapters/backup_backup_intro.tex <==
\section{Introduction}

\begin{figure}[!ht]
\begin{center}
\begin{tabular}{ c }
\includegraphics[width=0.95\linewidth]{latex/ICCV_2021/Figures/Images/Teaser_Figure/0_with_prediction.png}\\
\end{tabular}
\caption{{\bf Approximating the loss}. Training the network $f_{\Theta}(x)$ from scratch on a single image and its corresponding label map. On the right we see the label map produced by the trained network. (Top row) full supervision: The loss is computed on all pixels in the label map. (Bottom row) The loss is computed on less than ~$0.1$\% of the labeled pixels (pixels marked in red). Both networks achieve comparable, and sometimes indistinguishable, results. On average, labeling $0.03\%$ pixels per image on Pascal VOC benchmark is enough to reach full-supervision results.}
\label{fig:teaser}
\end{center}
\end{figure}


Semantic segmentation of images is a required step in many computer vision applications such as such as image editing, image understanding, medical image analysis and more. Despite extensive research, and great progress, it is still a challenge because of the large variability in image content. 

% Very often, to achieve high quality results, a specialized semantic segmentation training set must be created, which might be a daunting task. But is it really? 

Annotating a new data set of images is often reduced to a sequence of single image annotations.
For each image, the user interactively adds scribbles until she is satisfied with the segmentation proposed by the network.

A typical approach for annotating a new data set of images is to rely on standard image annotation tools, such as scribbles, to annotate images, and then semi-automatically segment them. Scribble-based approaches can be seen as a form of Active Learning (AL). The user makes a few scribbles, observes the results, and adds some more. Repeating this process over many images creates a large enough set to train a semantic segmentation network. 

The networks used in these tools are first trained on a data set with similar images for best performance, which leads to a chicken-and-egg problem. How do you bootstrap the process in case of a new data set of images that may not look similar to standard academic data sets?
This problem can occur in various sectors such as military, medical, or commercial.



% Our goal is to examine what it takes to train a neural network on a single image from scratch. In our experiments, the user is replaced with an Oracle that determines which pixels to scribble. Such an Oracle-based approach allows us to evaluate different ways to determine how many pixels should be annotated and find their spatial distribution in the image plane. 

Our goal is to examine what it takes to train a neural network on a single image from scratch. \daniel{Changed text: We do so by utilizing an Oracle which has access to the entire label image}. The key finding is that when training a network on a single image, the loss can be computed on a subset of the pixels. See Figure~\ref{fig:teaser} \daniel{the reference to the figure seems unrelated to the text}. The network is trained on a single image with the loss defined only on the pixels marked with red. Once trained, the network can create a remarkably well pseudo-label for the entire image. The network can be initialized with pre-trained weights from ImageNet ~\cite{deng2009imagenet}. We do {\em not} train the network beforehand on a data set of similar images to perform semantic segmentation.

We investigate three components that affect the training process. The first, of course, is the required number of labeled pixels and their location in the image plane. The second is whether we need to use pre-trained networks (i.e., a network that was pre-trained on ImageNet ~\cite{deng2009imagenet}), as opposed to initializing network weights with random values. Lastly, we also examine the importance of the order in which labeled pixels are introduced during training.

In our experiments, the user is replaced with an Oracle that determines which pixels to click. Such an Oracle-based approach allows us to evaluate different ways to address these questions systematically.

To address the first question, we use existing semantic segmentation data sets, for which the ground truth is known, and evaluate different methods to sample pixels to serve as annotated ``clicks''. We use labels only on the selected pixels to train a neural network for segmentation.

Because we train the network just for a single image, we can use the label of just a fraction of the pixels for the loss. In other words, we found that, on average, annotating less than $0.1\%$ of the pixels in an image is sufficient to compute the loss required to train the network to segment the image successfully. 

To answer the second question, we repeat the experiment using pre-trained networks as well as \daniel{'and' instead of 'as well as'?} a network that is initialized with random values and find that the accuracy gap is considerable when the number of labeled pixels is extremely low \daniel{extremely low' sound not so good..highly sparse?} but the gap shrinks quickly as their number grows.

Then, we repeat the experiments, only this time, we try different ways in which the clicks are presented during training. We find that different orders leads to significant variations in performance. This can be seen as yet another manifestation of Curriculum Learning.

Next, we investigate how to extend this approach to the annotation of an entire data set. A na\"ive extension of our findings above would be to annotate $0.1\%$ of the pixels in many, or all of the images, and use only them to train a network for the entire data set. However, we found that this did not work well, and took a different approach. 

\daniel{People found this paragraph to be confusing because maybe because of the 'but'} Instead, for each image, we use the single-image-network we trained in the previous step to find and annotate pixels, but use them to create pseudo-labels for the entire image. These pseudo-labels are sufficiently accurate to train a new network for the entire data set. 
% We found that using as little as $30\%$ of the images from the original training set gives good results with little degradation in accuracy compared to training with the full training set.

We found that, on average, using the labels of less than $0.05\%$ of the pixels per image is enough to reach full-supervision results. These conclusions also hold for a low-data regime where we use just a subset of the training images.

We demonstrate this on two very different types of data sets: the Pascal-VOC 2012 dataset ~\cite{pascal-voc-2012}, a popular instance segmentation benchmark, and Kvasir-SEG ~\cite{jha2021comprehensive}, a medical imaging binary segmentation set. 
\daniel{Changed text: We also ran our experiment on a large subset of images from long-tailed distribution ,ADE20K dataset ~\cite{zhou2017scene}, and saw similar results, although a bit higher (~$0.5\%$), as it contains significantly higher class diversity in each image, so more user clicks are needed. See supplemental for more details about this data set.}
To summarize, we make the following contributions:
\begin{itemize}
  \item Propose a plug-and-play single image annotation algorithm that can work with any network architecture.
  \item Suggest a method to quickly annotate an entire data set based on our single-image-annotation approach. \daniel{a bit misleading, to propose a 'method'}
  \item Run extensive experiments to validate our results on two, very different, real-world data sets.
\end{itemize}

% \daniel{ADE20k? do we want to point it out? added text to emphasize practical aspects of our work: }Although our work is more therotical, we believe that it can be used for practical aspects by enabling to quantify better the amount of effort needed in order to segment a new dataset, which can be more feasible than one can assume. Our work can be extended to using continuous scribbles that will reduce annotation burden \daniel{We need to be careful not to say that our method enables segmenting images more easily, but rather shed some light on the importance of pixel and can serve as a future work for further investigating such redundancies, in order to make the annotation process more effective}.
% We believe that our work can be of interest to the active-learning community as it gives an upper bound on the number of pixels needed in order to segment an image, up to an entire dataset.
% Also, an extension of our work can be used for other dense problems like optical-flow, depth estimation.
% We believe that the findings of the \emph{pixel-level} curriculum learning can be of help to other sparsely labeled data.


% As we wish to estimate the amount of information needed to train a network, without any prior knowledge, we wish to exploit the internal statistics of an image for this matter. We utilize the field of 'Deep Internal Learning', that has seen increasing interest lately \daniel{Add refs? If we want to keep it as a section}, to work on semantic segmentation. 

% \textbf{Contributions.}
% \daniel{A bit copied from the 10\% we don't need - contribution} This work shed some light on semantic redundancies in semantic segmentation, which in turn can be used in various fields (improving interactive segmentation by proposing the important regions to the user, applying more sophisticated training techniques on a sparse supervision to improve explainability, reducing computation cost and labeling efforts). We do it by identifying a subset of pixels that are \textit{informative}, such that knowing them will help recover the entire semantic label image. To the best of our knowledge, this is the first work to suggest a feasible solution to which highly sparse pixels are informative for the task of semantic segmentation.

% \daniel{A bit copied from the 10\% we don't need - contribution} We do not claim algorithmic contributions, but rather demonstrating the existence of pixels redundancies in semantic segmentation across different datasets. However, we hope that our findings can motivate further research into identifying additional redundancies and exploiting them for more efficient models, training or data-collection. Our findings may also be of interest to active learning community, as it provides an upper-bound on the best performance\footnote{\daniel{A bit copied from the 10\% we don't need - footnote} Suppose we discover about the existence of $k$ pixels in an image of size $n >> k$ that contains all of the \textit{information} of the image and can reach at least the same results as using all $n$ pixels. Then if our training procedure cannot reach the full supervision performance after selecting $k$ pixels, we know that there \textit{might} exists a better training procedure, as there exists a subset of size $k$ that can achieve full supervision performance.
% %Suppose we learn about existence of m samples in a dataset of size $n > m$ that can achieve the same test performance as a model trained with all $n$ samples. Then if our active learner cannot reach the full test performance after selecting $m$ samples, we know that there \textit{might} exist a better active learning algorithm, as the ideal subset of size $m$ can achieve full test accuracy
% }.


%-------------------------------------------------------------------------

% \begin{itemize}
%   \item Propose a plug-and-play single image annotation algorithm that can work with any network architecture.
  
%   'easy-to-implement' \daniel{plug and play? we need to emphasize that unlike other papers, our approach is straightforward and easy to validate} generic algorithm for uncovering the most "informative" pixels for the task of semantic segmentation.
%   \item Give a notion of 'Curriculum Learning' in the pixel level.
%   \item Run extensive experiments and validate our results on two, very different, real-world datasets.
%   \item Expand the concept of 'Deep Internal Learning' for semantic segmentation.
%   \item Increase explainability of segmentation networks training by uncovering some insights.
% \end{itemize}

